Molecular Dynamics Simulations of Anisotropic Particles Accelerated by Neural-Net Predicted Interactions

Rigid bodies, made of smaller composite beads, are commonly used to simulate anisotropic particles with molecular dynamics or Monte Carlo methods. To accurately represent the particle shape and to obtain smooth and realistic effective pair interactions between two rigid bodies, each body may need to contain hundreds of spherical beads. Given an interacting pair of particles, traditional MD methods calculate the inter-body distances between the beads of the rigid bodies within a certain distance. For a system containing many anisotropic particles, distance calculations are computationally costly and limit the attainable system size and simulation time. However, the effective interaction between two rigid particles only depends on the distance between their center of masses and their relative orientation. Therefore, a function directly mapping the center of mass distance and orientation to the interaction energy between the two rigid bodies, would completely bypass inter-bead distance calculations. It is challenging to derive such a general function analytically for most non-spherical rigid bodies. We have trained neural nets, powerful tools to fit nonlinear functions to complex datasets, to achieve this task. The pair configuration is taken as input and the energy, forces and torques between two rigid particles are predicted directly. We show that MD simulations of cubes and cylinders performed with forces and torques obtained from the gradients of the energy neural-nets quantitatively match traditional simulations that uses composite rigid bodies. Both structural quantities and dynamic measures are in agreement, while achieving up to 23 times speed up over traditional molecular dynamics, depending on hardware and system size. The method can, in principle, be applied to any irregular shape with any pair interaction, provided that sufficient training data can be obtained.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}

==> sections/section06.tex <==
\section{Mean Square Rotation Calculation } \label{sec:Mean Square Rotation Calculation }
The calculation follows directly from ~\citep{quat_distance}. The ``distance'' $\mathrm{d}$ between two orientations can be given by the following:
$$
d\left(\boldsymbol{q}_1, \boldsymbol{q}_2\right)=1.0-\left\langle\boldsymbol{q}_1, \boldsymbol{q}_2\right\rangle^2
$$

Where $\boldsymbol{q}$ is the unit quaternion that describes the orientation of the particle. The inner product of two unit quaternions is given by the following:
$$
\left\langle\boldsymbol{q}_1, \boldsymbol{q}_2\right\rangle=\left\langle q_1^s+q_1^i \boldsymbol{i}+q_1^j \boldsymbol{j}+q_1^k \boldsymbol{k}, q_2^s+q_2^i \boldsymbol{i}+q_2^j \boldsymbol{j}+q_2^k \boldsymbol{k}\right\rangle=q_1^s q_2^s+q_1^i q_2^i+q_1^j q_2^j+q_1^k q_2^k
$$

After calculating this ``orientational distance'' between the starting orientation and orientations at each future timestep of the same particle, we average the distances of particles in the box to get the mean squared orientation at different conditions. Apart from calculation of distance measure this is similar to mean square displacement calculations.
